Cluster Cepheids with High Precision Gaia Parallaxes, Low Zeropoint Uncertainties, and Hubble Space Telescope Photometry

We present HST photometry of 17 Cepheids in open clusters and their mean parallaxes from Gaia EDR3. These parallaxes are more precise than those from individual Cepheids (G<8 mag) previously used to measure the Hubble constant because they are derived from an average of >300 stars per cluster. Cluster parallaxes also have smaller systematic uncertainty because their stars lie in the range (G>13 mag) where the Gaia parallax calibration is most comprehensive. Cepheid photometry employed in the period--luminosity relation was measured using the same instrument(WFC3) and filters(F555W,F814W,F160W) as extragalactic Cepheids in SNIa hosts. We find no evidence of residual parallax offset in this magnitude range, zp=-3+/-4 muas, consistent with Lindegren:2021b and most studies. The Cepheid luminosity (P=10d, solar-metallicity) in the HST near-infrared, Wesenheit system derived from the cluster sample is M_{H,1}^W=-5.902+/-0.025 and -5.890+/-0.018 mag with or without simultaneous determination of a parallax offset, respectively. These results are similar to measurements from field Cepheids, confirming the accuracy of the Gaia parallaxes over a broad range of magnitudes. The SH0ES distance ladder calibrated solely from this sample gives H_0=72.8+/-1.3 and H_0=73.2+/-1.1 km/s/Mpc with or without offset marginalization; combined with all anchors we find H_0=73.01+/-0.99 and 73.15+/-0.97, respectively, a 5% or 7% reduction in the uncertainty and a 5.3 sigma Hubble Tension relative to Planck+LambdaCDM. It appears increasingly difficult to reconcile two of the best measured cosmic scales, parallaxes from Gaia and the angular size of the acoustic scale of the CMB, using the simplest form of LambdaCDM to join the two.

==> figs_cluster.tex <==
\begin{figure}[ht]
\vspace*{150mm}
\figurenum{1}
\special{psfile=comp_hist.ps vscale=70 hscale=70 hoffset=530 voffset=-20 angle=90}
\caption{\label{fg:outlier}  Sources used by L20 to calibrate the \Gaia EDR3 parallax offset (LMC stars and QSOs) and samples used to measure the parallaxes of Cepheids.  L20 also used $\sim$ 7000 physical pairs of stars (not in this plot) with the brighter member having $6 < G < 10$ to calibrate the bright range.  The parallaxes of field Cepheids (blue line) used in R21 and the SH0ES determination of $H_0$ require the simultaneous determination of the parallax offset due to the more limited \Gaia calibration in this range.  The parallaxes of Cepheids in clusters were determined with a far greater number of stars which are also fainter (green), in the brightness range where \Gaia is best calibrated. The dotted line (upper) shows the fiducial luminosity calibration.}
\end{figure}


\begin{figure}[ht]
\vspace*{150mm}
\figurenum{2}
\special{psfile=show_pl_new1.ps vscale=70 hscale=70 hoffset=530 voffset=-20 angle=90}
\caption{\label{fg:outlier}  The Milky Way Cepheid period-luminosity relation in the {\it HST} NIR, reddening Free (Wesenheit) system as calibrated with three samples.  Parallaxes from {\it HST} spatial scanning (R18) for 8 Cepheids are in blue and yield 3\% precision.  The 68 points in gray (R21) using \Gaia EDR3 parallaxes with simultaneous calibration of the parallax offset.  The red points come from cluster Cepheids and do not require parallax offset calibration as they are measured in the range where \Gaia is best calibrated.  These samples differ in their parallax precision (inset) leading to the low dispersion of $\sigma=0.07$ mag for the cluster Cepheids.}
\end{figure}



